Quantum phase fluctuations quench chiral superconductivity in twisted overdoped cuprate bilayers

Twisted cuprate bilayers have been proposed to host chiral superconductivity at temperatures comparable to their large pairing scale, yet experimental signatures of broken time-reversal symmetry remain unclear. We show that quantum phase fluctuations strongly suppress chiral order in twisted overdoped cuprate bilayers despite robust intralayer pairing. At a $45^\circ$ twist, we analytically demonstrate that the chiral transition temperature obeys $T_\chi\propto t^4$ when the single-electron interlayer tunneling amplitude $t$ is weak. This collapse originates from competition between the small Josephson energy scale supporting chirality and the temperature-dependent collective zero-point energy. Chirality consequently survives only in a narrow angular window at ultralow temperatures, with relative-phase plasma softening above the chiral transition. A distinct transport signature arising from the quantum phase fluctuations is a pronounced low-temperature enhancement of the critical current near a magic angle. These findings separate pairing and chiral ordering scales and offer a possible explanation for the difficulty of observing robust chiral superconductivity in twisted cuprates.

==> arxiv-layout.tex <==
% Layout-only adaptation for one self-contained arXiv PDF.
\makeatletter
\AtBeginDocument{%
  \let\arxiv@hangfrom@section\@hangfrom@section
  \let\arxiv@sectioncntformat\@sectioncntformat
}
\newcommand{\arxivStartSupplement}{%
  \clearpage
  \onecolumngrid
  \thispagestyle{titlepage}%
  \setcounter{page}{1}%
  \renewcommand{\thepage}{S\arabic{page}}%
  \setcounter{section}{0}%
  \setcounter{subsection}{0}%
  \setcounter{subsubsection}{0}%
  \setcounter{equation}{0}%
  \setcounter{figure}{0}%
  \setcounter{table}{0}%
  % End Matter's appendix setup otherwise resets equations at each section.
  \counterwithout*{equation}{section}%
  \let\@hangfrom@section\arxiv@hangfrom@section
  \let\@sectioncntformat\arxiv@sectioncntformat
  \renewcommand{\thesection}{S\arabic{section}}%
  \renewcommand{\thesubsection}{\thesection.\arabic{subsection}}%
  \renewcommand{\p@subsection}{}%
  \renewcommand{\theequation}{S\arabic{equation}}%
  \renewcommand{\thefigure}{S\arabic{figure}}%
  \renewcommand{\thetable}{S\arabic{table}}%
  % Distinct PDF destinations are essential when counters restart.
  \renewcommand{\theHsection}{S\arabic{section}}%
  \renewcommand{\theHsubsection}{\theHsection.\arabic{subsection}}%
  \renewcommand{\theHequation}{S\arabic{equation}}%
  \renewcommand{\theHfigure}{S\arabic{figure}}%
  \renewcommand{\theHtable}{S\arabic{table}}%
  \setcounter{secnumdepth}{2}%
  \setcounter{tocdepth}{2}%
  \allowdisplaybreaks[1]%
  % Only Supplemental headings go into the Supplemental contents file.
  \let\arxiv@addcontentsline\addcontentsline
  \renewcommand{\addcontentsline}[3]{%
    \def\arxiv@extension{##1}\def\arxiv@toc{toc}%
    \ifx\arxiv@extension\arxiv@toc
      \arxiv@addcontentsline{stc}{##2}{##3}%
    \else
      \arxiv@addcontentsline{##1}{##2}{##3}%
    \fi
  }%
  \phantomsection
  \def\@currentlabel{}%
  \label{S-supplement-start}%
  \pdfbookmark[0]{Supplemental Material}{supplement}%
}
\newcommand{\arxivSupplementTitle}[2]{%
  \vspace*{-14pt}%
  {\centering\large\bfseries #1\par}%
  \vspace{12.5pt}%
  {\centering\normalsize #2\par}%
  \vspace{27pt}%
}
\newcommand{\arxivSupplementContents}{%
  \addtocontents{stc}{\string\tocdepth@munge}%
  \begingroup
    \section*{\tocname}%
    \let\appendix\appendix@toc
    \@starttoc{stc}%
  \endgroup
  \addtocontents{stc}{\string\tocdepth@restore}%
}
\makeatother

